TRIDEnT: Building Decentralized Incentives for Collaborative Security

Sophisticated mass attacks, especially when exploiting zero-day vulnerabilities, have the potential to cause destructive damage to organizations and critical infrastructure. To timely detect and contain such attacks, collaboration among the defenders is critical. By correlating real-time detection information (alerts) from multiple sources (collaborative intrusion detection), defenders can detect attacks and take the appropriate defensive measures in time. However, although the technical tools to facilitate collaboration exist, real-world adoption of such collaborative security mechanisms is still underwhelming. This is largely due to a lack of trust and participation incentives for companies and organizations. This paper proposes TRIDEnT, a novel collaborative platform that aims to enable and incentivize parties to exchange network alert data, thus increasing their overall detection capabilities. TRIDEnT allows parties that may be in a competitive relationship, to selectively advertise, sell and acquire security alerts in the form of (near) real-time peer-to-peer streams. To validate the basic principles behind TRIDEnT, we present an intuitive game-theoretic model of alert sharing, that is of independent interest, and show that collaboration is bound to take place infinitely often. Furthermore, to demonstrate the feasibility of our approach, we instantiate our design in a decentralized manner using Ethereum smart contracts and provide a fully functional prototype.

==> privacy.tex <==
\smallskip\par\noindent\textbf{Privacy concerns. }
In this first version of \textit{TRIDEnT}, we offer increased privacy assurances for participants by allowing the formation
of P2P overlays based on trust, i.e. alert data is not published indiscreetly. Solutions offering anonymous payments and privacy-preserving reputation (e.g.,~\cite{schaub2016trustless})
could be integrated into our design, but are out of the scope of this paper. Alerts are assumed to be sanitized according to best practices (e.g.,\cite{lincoln2004privacy}).


==> proofs.tex <==
%\section{Markov chain of attacker behavior}\label{app:markov}
%Figure to aid understanding of the model of Section~\ref{sec:model}.
%\begin{figure}[h]
%	\centering
%	%\begin{minipage}{4in}
%	\begin{tikzpicture}[shorten >=1pt,node distance=4cm, auto]
%	\node[state] (nn) {$\neg a,\neg a$};
%	\node[state] (an) [right of = nn] {$a,\neg a$};
%	\node[state] (na) [below of = nn]{$\neg a, a$};
%	\node[state] (aa) [below of = an]{$a, a$};
%	
%	\path[->] (nn) edge [bend left] node [above] {$p-p^2$} (an)
%	(an) edge node [above] {$(1-q)^2$} (nn)
%	(an) edge [bend left = 40] node [right] {$q^2$} (aa)
%	(aa) edge  [bend left = 20] node [right] {$q-q^2$} (an)
%	(nn) edge [bend left = 20] node [left] {$p-p^2$} (na)
%	(na) edge  [bend left = 40] node [left] {$(1-q)^2$} (nn)
%	(na) edge node [below] {$q^2$} (aa)
%	(aa) edge  [bend left] node [below] {$q-q^2$} (na) 
%	(nn) edge [bend left = 15] node [near end, below] {$p^2$} (aa)
%	(aa) edge [bend left = 15] node [near end, above] {$(1-q)^2$} (nn)
%	(aa) edge  [bend left] node [below] {$q-q^2$} (na);
%	\draw [<->]	(na) edge  node [near start, below] {$q-q^2$} (an);
%	\end{tikzpicture}
%	\caption{Markov chain example depicting the attacker's behavior (self loops are not displayed).}
%	\label{fig:aMC1}
%	%\end{minipage}
%	%\begin{minipage}{2in}
%	%\begin{tikzpicture}[shorten >=1pt,node distance=3.5cm, auto]
%	% \node[state] (n) {$\neg a,\neg a$};
%	%  \node[state] (a) [right of = nn] {$\begin{array}{c}a,\neg a\\\neg a, a\\a,a\end{array}$};
%	%
%	%\path[->] (n) edge [bend left] node [above] {$p(2-p)$} (a)
%	% 		(n) edge [loop above] node [above] {$(1-p)^2$}(n)
%	%		(a) edge [bend left] node [below] {$(1-q)^2$} (n)
%	%		(a) edge [loop above] node [above] {$q(2-q)$}(a);
%	%		 \end{tikzpicture}
%	%\caption{}
%	%\label{fig:aMC2}
%	%\end{minipage}
%	% \caption{}
%	%\label{fig:}
%\end{figure}
\section{Proofs}
\subsection{Proof of Lemma~\ref{lem:length-cycle}}\label{app:lem-cycle}
\begin{proof}
	$E(L_a) = \sum_{0}^{+\infty} n \p(L_a = n) = \sum_{0}^{+\infty} n q^n(1-q) = \frac{1}{1-q}$.\\ $E(L_{\neg a}) = \sum_{0}^{+\infty} n \p(L_{\neg a} = n) \leq \sum_{0}^{+\infty} n (1-p)^nq = \frac{q(1-p)}{p^2} + 1$.
\end{proof}
\subsection{Proof of Theorem~\ref{lem:buy-NE}}\label{app:theorem1proof}
\begin{proof} We prove the last statement.
		
		The first time that Player $0$ is not attacked is either after the first occurrence of the pattern $A^0_{n-1} = a \wedge A^0_n = \neg a$ or at time $0$, which is as if $A^0_{n-1} = a \wedge A^0_n = \neg a$ had just occurred (since Attacker uses probability $q$ at the beginning.) Since $\delta < q \alpha$, this is first time that Player $0$ may need information. At this time Player $0$ would buy information iff $s^1 \leq \min(q\alpha - \delta, \frac{1-q}{q}(\delta - p\alpha))$. Note that purchase occurs also for $s^1 = \min(q\alpha - \delta, \frac{1-q}{q}(\delta - p\alpha)))$ since the two options give the same expected instant cost, but buying the information may be also useful for future rounds (which is beyond the scope of this paper). Therefore the optimal value of $s^1$ (for Player $1$) is $\min(q\alpha - \delta, \frac{1-q}{q}(\delta - p\alpha))$. Likewise, this is also the optimal value of $s^0$.
	\end{proof}

